UniDiffFusion: A Unified Diffusion Framework for Multi-Task and Degradation-Robust Image Fusion

General image fusion aims to integrate complementary information from multiple source images, but existing methods often rely on task-specific models and struggle to maintain robust performance under diverse degradation conditions. In this paper, we propose UniDiffFusion, a unified diffusion framework for multi-task and degradation-robust image fusion. UniDiffFusion leverages the strong generative prior of a pretrained diffusion model to establish a shared fusion backbone across heterogeneous fusion tasks, while introducing task- and degradation-aware conditional adaptation to accommodate their distinct information-selection requirements. Specifically, we employ task prompt modulation to progressively adapt the shared diffusion representations to different fusion objectives, and develop a degradation prompt router to dynamically retrieve degradation-aware priors and restore corrupted source features before fusion. Furthermore, an application prompt bank is introduced to incorporate task-oriented semantic guidance for downstream applications, such as object detection and semantic segmentation, without altering the shared fusion and restoration pathways. The proposed framework is trained in a progressive manner to decouple fusion learning, degradation-aware restoration, and application-specific adaptation, thereby reducing interference among heterogeneous objectives. Extensive experiments on visible-infrared, multi-exposure, and multi-focus image fusion demonstrate that UniDiffFusion achieves superior fusion quality and robustness under both clean and degraded conditions. Moreover, UniDiffFusion consistently improves downstream detection and semantic segmentation performance, demonstrating its effectiveness as a unified diffusion framework for both perceptual fusion and task-oriented vision.

==> sec/3_method_bak.tex <==

\section{Method}
\label{sec:method}
\subsection{Framework Overview}
\label{sec:method_overview}
Unlike the application identity, which is manually specified when downstream adaptation is required, the fusion task and degradation conditions are inferred internally from the input representations. Accordingly, the unified fusion process is formulated as
\begin{equation}
    \mathbf{y}= \mathcal{G}_{\Theta}
    \left(
        \mathbf{x}^{1},
        \mathbf{x}^{2};
        a
    \right),
    \qquad
    a\in\mathcal{A}\cup\{\varnothing\},
    \label{eq:problem_formulation}
\end{equation}
where task- and degradation-aware adaptation is performed automatically by TPM and DPR, respectively.

As illustrated in Fig.~\ref{fig:framework}, HP-UniIF is built on a pretrained latent diffusion model comprising a variational autoencoder (VAE) and a denoising U-Net. For each source image, the VAE encoder extracts a latent code together with hierarchical intermediate features:
\begin{equation}
    \left(
        \mathbf{z}^{i},
        \{\mathbf{s}^{i}_{l}\}_{l=1}^{L}
    \right)
    =
    \mathcal{E}(\mathbf{x}^{i}),
    \qquad
    i\in\{1,2\},
    \label{eq:source_encoding}
\end{equation}
where $\mathbf{z}^{i}$ denotes the latent representation and $\mathbf{s}^{i}_{l}$ is the intermediate feature extracted at encoder level $l$.

The source latents are first aggregated through a learnable convolutional projection:
\begin{equation}
    \mathbf{z}^{f}=F_{z}\!\left([\mathbf{z}^{1};\mathbf{z}^{2}]\right)
    \label{eq:latent_fusion}
\end{equation}
where $[\cdot;\cdot]$ denotes channel-wise concatenation. The fused latent $\mathbf{z}^{f}$ is then progressively refined through $T$ denoising steps to yielding the clean latent representation $\mathbf{z}_{0}$. 

Subsequently, $\mathbf{z}_{0}$ is decoded together with the hierarchical source features in a coarse-to-fine manner. The decoding process at level $l$ can be expressed as $h_l=\mathcal{D}(z_0, \{s\}_l^i)$. 
% At each decoder level, DPR first identifies the degradation condition and retrieves the corresponding prompts to restore corruption-affected representations. TPM then infers a soft fusion-task condition and adaptively modulates the restored features according to the current fusion objective. Finally, APB introduces the specified application condition while preserving the source evidence required for faithful and task-relevant fusion. The progressively refined representation is subsequently mapped to the final fused image through the VAE decoder.
% The three modules therefore address complementary dimensions of unified fusion. DPR improves robustness to heterogeneous input degradations, TPM adapts source selection and combination to different fusion objectives, and APB emphasizes application-relevant evidence without discarding fusion-essential content. Together, they enable a shared generative backbone to accommodate diverse fusion tasks, degradation conditions, and downstream applications.
% \subsection{Task Prompt Modulation}
\label{sec:tpm}

Different fusion tasks require distinct source-selection and information-preservation behaviors. 
% MIF emphasizes thermal saliency while preserving visible textures, MEF balances informative regions across different exposure levels, and MFF selects locally focused structures. 
Consequently, directly sharing a static fusion operator across all tasks may lead to task-agnostic feature aggregation and compromise task-specific fusion quality. 
TPM infers a task condition from the current source and decoder representations and uses it to adapt feature fusion at each decoder level. Let $\widetilde{\mathbf{s}}^{i}_{l}$ denote the source feature restored by DPR. We first aggregate the restored source features with the incoming decoder representation:
\begin{equation}
    \mathbf{u}^{t}_{l}=\mathcal{C}^{t}_{l}
    \left(
        [\widetilde{\mathbf{s}}^{1}_{l};
         \widetilde{\mathbf{s}}^{2}_{l}]
    \right)
    +
    \mathcal{U}^{t}_{l}
    \left(
        \mathbf{h}_{l+1}
    \right),
    \label{eq:tpm_feature_aggregation}
\end{equation}
where $\mathcal{C}^{t}_{l}$ denotes a convolutional projection and
$\mathcal{U}^{t}_{l}$ performs spatial upsampling and channel alignment.
A compact task descriptor is subsequently obtained by
\begin{equation}
    \mathbf{q}^{t}_{l} = \operatorname{MLP}(\operatorname{GAP}(\mathbf{u}^{t}_{l})).
    \label{eq:tpm_task_descriptor}
\end{equation}
here, $\mathbf{W},\mathbf{B}$ is a MLP project.
At decoder level $l$, TPM maintains a learnable prompt embedding $\mathbf{P}^{t}_{l}$
where each row denotes a task-oriented prompt basis.
The soft routing formulation provides a differentiable task-conditioning mechanism and allows the decoder to adapt to intra-task variations in the source representations.

The retrieved prompt is jointly encoded with the current feature descriptor to generate channel-wise modulation parameters:
\begin{equation}
    \left(
        \boldsymbol{\gamma}^{t}_{l},
        \boldsymbol{\beta}^{t}_{l},
        \mathbf{g}^{t}_{l}
    \right)
    =
    \operatorname{MLP}^{t}_{l}
    \left(
        [\mathbf{q}^{t}_{l};
         \mathbf{p}^{t}_{l}]
    \right).
    \label{eq:tpm_modulation_parameters}
\end{equation}
The task-adapted feature is computed through gated residual modulation:
\begin{equation}
    \widehat{\mathbf{u}}^{t}_{l}
    =
    \mathbf{u}^{t}_{l}
    +
    \sigma
    \left(
        \mathbf{g}^{t}_{l}
    \right)
    \odot
    \left(
        \boldsymbol{\gamma}^{t}_{l}
        \odot
        \mathbf{u}^{t}_{l}
        +
        \boldsymbol{\beta}^{t}_{l}
    \right),
    \label{eq:tpm_feature_modulation}
\end{equation}
where
$\boldsymbol{\gamma}^{t}_{l},
\boldsymbol{\beta}^{t}_{l},
\mathbf{g}^{t}_{l}\in\mathbb{R}^{C_l}$
are broadcast along the spatial dimensions. The identity pathway retains
the shared feature representation, while the sigmoid gate adaptively
controls the magnitude of the task-conditioned residual.
% Applying TPM throughout the decoder enables task conditioning at multiple spatial scales. Coarse-resolution stages facilitate global source coordination, whereas finer stages refine local task-dependent details. This hierarchical modulation allows HP-UniIF to share a common generative backbone while preserving task-specific fusion behavior.

% \subsection{Degradation Prompt Router}
% \label{sec:dpr}

% % Inputs in the 3M setting may suffer from unknown or compound degradations whose from unknown or compound degradations whose characteristics vary across samples, source modalities, and feature scales. A fixed degradation embedding is therefore insufficient to provide adaptive restoration guidance. DPR addresses this issue by retrieving reusable degradation patterns from a learnable prompt pool and complementing them with an input-dependent prompt. The resulting condition jointly guides latent recovery and hierarchical feature restoration.
% DPR retrieves reusable degradation patterns from a learnable prompt pool and complements them with an input-dependent prompt. The resulting condition jointly guides latent recovery and hierarchical feature restoration.
% At decoder level $l$, DPR first constructs a compact degradation descriptor from the two source features and the incoming decoder representation:
% \begin{equation}
%     \mathbf{a}^{d}_{l}=\operatorname{GAP}(\mathcal{C}^{d}_{l}
%         (
%             [
%                 \mathbf{s}^{1}_{l};
%                 \mathbf{s}^{2}_{l};
%                 |\mathbf{s}^{1}_{l}-\mathbf{s}^{2}_{l}|;
%                 \mathcal{U}^{d}_{l}(\mathbf{h}_{l+1})
%             ]
%         )
%     ),
%     \label{eq:dpr_descriptor}
% \end{equation}
% where $\mathcal{U}^{d}_{l}$ aligns the decoder feature with the current source features, and $\mathcal{C}^{d}_{l}$ denotes a convolutional projection. The feature discrepancy provides an explicit cue for source-dependent corruption and inconsistency.

% DPR maintains a level-specific prompt pool containing $N_p$ learnable key-value pairs, and a normalized retrieval query is predicted from the degradation descriptor:
% \begin{equation}
%     \mathcal{I}_{l}=\operatorname{TopK}(\operatorname{Norm}(Q^{d}_{l}(\mathbf{a}^{d}_{l})
% \cdot(\mathbf{K}^{d}_{l})^{\top}, K).
%     \label{eq:dpr_topk}
% \end{equation}
% where $Q^{d}_{l}$ is a learnable projection. Based on the similarity between the query and prompt keys, DPR selects the $K$ most relevant entries:
% The retrieved prompt is computed as a weighted combination of the selected
% prompt values:
% \begin{equation}
%     \mathbf{p}^{r}_{l}=\sum_{j\in\mathcal{I}_{l}}   \omega^{d}_{l,j}\mathbf{p}^{d}_{l,j},
%     \qquad
%     \omega^{d}_{l,j}
%     =
%     \frac{
%         \exp(r^{d}_{l,j}/\tau_d)
%     }{
%         \sum_{m\in\mathcal{I}_{l}}
%         \exp(r^{d}_{l,m}/\tau_d)
%     },
%     \label{eq:dpr_retrieval}
% \end{equation}
% where $r^{d}_{l,j}=(\mathbf{q}^{d}_{l})^{\top} \operatorname{Norm}(\mathbf{k}^{d}_{l,j})$ and $\tau_d$ is a temperature parameter.

% Inspired by~\cite{vaishnav2023promptir}, we design a feature-guided prompting mechanism that captures sample-specific corruption severity and spatially varying degradation patterns, thereby generating content-adaptive prompts.
% \begin{equation}
%     \mathbf{p}^{g}_{l}=G^{d}_{l}(\mathbf{a}^{d}_{l}) \\
%     \mathbf{c}^{d}_{l} = F^{d}_{l}([\mathbf{p}^{r}_{l};\mathbf{p}^{g}_{l}]),
%     \label{eq:dpr_prompt_fusion}
% \end{equation}
% where $G^{d}_{l}$ denotes the prompt generator and $F^{d}_{l}$ fuses the
% retrieved and generated prompts. Thus, $\mathbf{c}^{d}_{l}$ combines
% reusable restoration knowledge with input-adaptive degradation information.
% The fused degradation condition is mapped to source-specific modulation
% parameters:
% \begin{equation}
%     \left(
%         \boldsymbol{\gamma}^{d,i}_{l},
%         \boldsymbol{\beta}^{d,i}_{l},
%         \mathbf{g}^{d,i}_{l}
%     \right)
%     =
%     H^{d,i}_{l}
%     \left(
%         \mathbf{c}^{d}_{l}
%     \right),
%     % \qquad
%     % i\in\{1,2\}.
%     \label{eq:dpr_parameters}
% \end{equation}
% The restored source features are obtained through gated residual modulation:
% \begin{equation}
%     \widetilde{\mathbf{s}}^{i}_{l}
%     =
%     \mathbf{s}^{i}_{l}
%     +
%     \sigma(\mathbf{g}^{d,i}_{l})
%     \odot
%     \left(
%         \boldsymbol{\gamma}^{d,i}_{l}
%         \odot
%         \mathcal{N}^{d,i}_{l}(\mathbf{s}^{i}_{l})
%         +
%         \boldsymbol{\beta}^{d,i}_{l}
%     \right),
%     \label{eq:dpr_feature_restoration}
% \end{equation}
% where $\mathcal{N}^{d,i}_{l}$ is a lightweight restoration transform and the channel-wise parameters are broadcast along the spatial dimensions. The identity pathway retains source evidence, while the learned gate controls the magnitude of degradation-aware correction. The restored features are subsequently passed to TPM for task-conditioned fusion.

% DPR also converts the multi-scale conditions
% $\{\mathbf{c}^{d}_{l}\}_{l=1}^{L}$ into control features for the frozen
% denoising U-Net:
% \begin{equation}
%     \widehat{\boldsymbol{\epsilon}}_{n} =U_{\theta}(\mathbf{z}_{n},n;C_{\phi}
%         (
%             \mathbf{z}_{n},
%             \{\mathbf{c}^{d}_{l}\}_{l=1}^{L}
%         )
%     ),
%     \label{eq:dpr_latent_control}
% \end{equation}
% where $C_{\phi}$ is a lightweight controller following
% SCEdit~\cite{jiang2024scedit}. Consequently, the same degradation
% representation coordinates global latent recovery and local multi-scale
% feature restoration.



\subsection{Task Prompt Modulation}
\label{sec:tpm}
Different fusion tasks require distinct information-selection and
preservation behaviors. For example, infrared--visible fusion emphasizes cross-modal complementarity, whereas multi-exposure and multi-focus fusion favor exposure-aware and focus-aware source selection, respectively. Task Prompt Modulation (TPM) therefore introduces a task-conditioned prompt that progressively adapts the shared latent and decoder representations to the current fusion objective.

For each fusion task $t\in\mathcal{T}$, TPM maintains a learnable prompt embedding:
\begin{equation}
    \mathbf{P}^{T}
    =
    [
        \mathbf{p}^{T}_{1};
        \ldots;
        \mathbf{p}^{T}_{|\mathcal{T}|}
    ]
    \in
    \mathbb{R}^{|\mathcal{T}|\times d_t},
    \qquad
    \mathbf{p}^{T}_{0}
    =
    \mathbf{P}^{T}[t],
    \label{eq:tpm_prompt_initialization}
\end{equation}
where $\mathbf{p}^{T}_{0}$ initializes the task condition and is subsequently
propagated across the latent, decoder, and output stages.

At decoder level $l$, the restored source features produced by DPR are first
fused and combined with the incoming decoder representation:
\begin{equation}
    \mathbf{u}^{T}_{l}
    =
    \mathcal{C}^{f}_{l}
    \left(
        [
            \widetilde{\mathbf{s}}^{1}_{l};
            \widetilde{\mathbf{s}}^{2}_{l}
        ]
    \right)
    +
    \mathcal{U}^{T}_{l}
    \left(
        \mathbf{h}_{l+1}
    \right),
    \label{eq:tpm_feature_aggregation}
\end{equation}
where $\mathcal{C}^{f}_{l}$ performs cross-source skip fusion and
$\mathcal{U}^{T}_{l}$ aligns the incoming decoder feature to the current
spatial resolution.

Rather than using a fixed task embedding throughout the decoder, TPM updates
the prompt according to the current feature state. A compact feature
descriptor is first extracted as
\begin{equation}
    \mathbf{q}^{T}_{l}
    =
    \Phi^{T}_{l}
    \left(
        \operatorname{GAP}
        \left(
            \mathbf{u}^{T}_{l}
        \right)
    \right),
    \label{eq:tpm_feature_descriptor}
\end{equation}
where $\Phi^{T}_{l}$ denotes a lightweight projection. The incoming prompt is
then refined using the feature descriptor and a learnable stage token
$\mathbf{e}^{T}_{l}$:
\begin{equation}
    \mathbf{p}^{T}_{l}
    =
    \mathbf{p}^{T}_{l+1}
    +
    R^{T}_{l}
    \left(
        [
            \mathbf{p}^{T}_{l+1}
            +
            \mathbf{e}^{T}_{l};
            \mathbf{q}^{T}_{l}
        ]
    \right),
    \label{eq:tpm_prompt_refinement}
\end{equation}
where $R^{T}_{l}$ is a prompt-refinement network. This recurrent update allows
the task condition to evolve from coarse semantic representations to
fine-grained spatial details.

The refined prompt predicts channel-wise affine parameters and an injection
gate:
\begin{equation}
    \left(
        \boldsymbol{\gamma}^{T}_{l},
        \boldsymbol{\beta}^{T}_{l},
        \mathbf{g}^{T}_{l}
    \right)
    =
    M^{T}_{l}
    \left(
        \mathbf{p}^{T}_{l}
    \right).
    \label{eq:tpm_modulation_parameters}
\end{equation}
The task-adapted feature is obtained through bounded gated residual
modulation:
\begin{equation}
    \widehat{\mathbf{u}}^{T}_{l}
    =
    \mathbf{u}^{T}_{l}
    +
    \sigma
    \left(
        \mathbf{g}^{T}_{l}
    \right)
    \odot
    \left[
        \rho_l
        \tanh
        \left(
            \boldsymbol{\gamma}^{T}_{l}
        \right)
        \odot
        \mathbf{u}^{T}_{l}
        +
        \rho_l
        \tanh
        \left(
            \boldsymbol{\beta}^{T}_{l}
        \right)
    \right],
    \label{eq:tpm_feature_modulation}
\end{equation}
where $\rho_l$ is a small residual scale, and all channel-wise parameters are
broadcast along the spatial dimensions. The identity pathway preserves the
shared representation, while the bounded affine transformation and sigmoid
gate prevent excessive task-specific perturbations.

The same feature-guided modulation is applied to the fused latent before
decoding and to the final output representation, with stage-specific
parameters and tokens. The updated prompt is passed sequentially across these
stages, enabling consistent task conditioning throughout the generation
process. Consequently, TPM adapts the shared backbone to different fusion
objectives while retaining a compact and stable task-specific modulation
path.

\subsection{Degradation Prompt Router}
\label{sec:dpr}

Input degradations may corrupt source features differently across modalities
and spatial scales, making direct skip fusion prone to propagating unreliable
information into the decoder. To address this issue, the Degradation Prompt
Router (DPR) restores the two source skip features before they are fused at
each decoder level. Specifically, DPR retrieves reusable degradation patterns
from a learnable prompt pool and combines them with an input-adaptive prompt
to guide gated feature correction.

At decoder level $l$, DPR estimates the degradation condition from the two
source skip features and the incoming decoder representation:
\begin{equation}
    \mathbf{a}^{d}_{l}
    =
    \operatorname{GAP}
    \left(
        \mathcal{C}^{d}_{l}
        \left(
            [
                \mathbf{s}^{1}_{l};
                \mathbf{s}^{2}_{l};
                |\mathbf{s}^{1}_{l}-\mathbf{s}^{2}_{l}|;
                \mathcal{U}^{d}_{l}(\mathbf{h}_{l+1})
            ]
        \right)
    \right),
    \label{eq:dpr_descriptor}
\end{equation}
where $\mathcal{U}^{d}_{l}$ aligns the incoming decoder feature with the
current skip features, and $\mathcal{C}^{d}_{l}$ denotes a convolutional
projection. The cross-source discrepancy provides an explicit cue for
modality-dependent corruption, while $\mathbf{h}_{l+1}$ supplies contextual
information from the coarser decoder stage.

DPR maintains a level-specific prompt pool
$\{(\mathbf{k}^{d}_{l,j},\mathbf{p}^{d}_{l,j})\}_{j=1}^{N_p}$.
A normalized query
\begin{equation}
    \mathbf{q}^{d}_{l}
    =
    \operatorname{Norm}
    \left(
        Q^{d}_{l}(\mathbf{a}^{d}_{l})
    \right)
\end{equation}
is used to retrieve the $K$ most relevant prompt entries. The resulting
retrieval prompt is
\begin{equation}
    \mathbf{p}^{r}_{l}
    =
    \sum_{j\in\mathcal{I}_{l}}
    \omega^{d}_{l,j}\mathbf{p}^{d}_{l,j},
    \qquad
    \omega^{d}_{l,j}
    =
    \frac{
        \exp(r^{d}_{l,j}/\tau_d)
    }{
        \sum_{m\in\mathcal{I}_{l}}
        \exp(r^{d}_{l,m}/\tau_d)
    },
    \label{eq:dpr_retrieval}
\end{equation}
where
$r^{d}_{l,j}
=
(\mathbf{q}^{d}_{l})^{\top}
\operatorname{Norm}(\mathbf{k}^{d}_{l,j})$,
$\mathcal{I}_{l}
=
\operatorname{TopK}(\{r^{d}_{l,j}\}_{j=1}^{N_p},K)$,
and $\tau_d$ is a temperature parameter.

To complement the reusable degradation patterns with sample-specific information, DPR generates an input-adaptive prompt and combines it with the retrieved prompt:
\begin{equation}
    \mathbf{p}^{g}_{l}
    =
    G^{d}_{l}(\mathbf{a}^{d}_{l}),
    \qquad
    \mathbf{c}^{d}_{l}
    =
    F^{d}_{l}
    \left(
        [\mathbf{p}^{r}_{l};\mathbf{p}^{g}_{l}]
    \right),
    \label{eq:dpr_prompt_fusion}
\end{equation}
where $\mathbf{c}^{d}_{l}$ encodes both reusable restoration knowledge and
input-dependent degradation characteristics.

Conditioned on $\mathbf{c}^{d}_{l}$, a lightweight restoration transform
predicts a source-specific correction
$\Delta\mathbf{s}^{d,i}_{l}$ and its injection gate
$\mathbf{g}^{d,i}_{l}$. The restored skip feature is written compactly as
\begin{equation}
    \widetilde{\mathbf{s}}^{i}_{l}
    =
    \mathbf{s}^{i}_{l}
    +
    \sigma(\mathbf{g}^{d,i}_{l})
    \odot
    \Delta\mathbf{s}^{d,i}_{l},
    \qquad
    \left(
        \Delta\mathbf{s}^{d,i}_{l},
        \mathbf{g}^{d,i}_{l}
    \right)
    =
    R^{d,i}_{l}
    \left(
        \mathbf{s}^{i}_{l},
        \mathbf{c}^{d}_{l}
    \right),
    \label{eq:dpr_feature_restoration}
\end{equation}
where $R^{d,i}_{l}$ denotes the prompt-conditioned restoration block. The
identity pathway preserves reliable source evidence, while the learned gate
controls how much degradation-aware correction is introduced.

Finally, the two restored skip features are fused and delivered to the
subsequent task-adaptive decoder:
\begin{equation}
    \mathbf{f}_{l}
    =
    \mathcal{C}^{f}_{l}
    \left(
        [
            \widetilde{\mathbf{s}}^{1}_{l};
            \widetilde{\mathbf{s}}^{2}_{l}
        ]
    \right).
    \label{eq:dpr_skip_fusion}
\end{equation}
By operating before skip-feature fusion, DPR suppresses degradation-induced interference while retaining complementary source information for subsequent task-conditioned modulation.


\subsection{Application Prompt Bank}
\label{sec:apb}

% Although the preservation of complementary source information primarily determines fusion quality, different downstream applications may favor different visual evidence. However, directly optimizing the entire fusion network with application objectives may distort low-level intensity, texture, and structural information. APB therefore introduces application-specific adaptation through a compact prompt bank.
APB introduces application-specific adaptation through a compact prompt bank.

We construct a learnable application prompt bank
\begin{equation}
    \mathbf{E}
    =
    [
        \mathbf{e}^{a}_{1};
        \mathbf{e}^{a}_{2};
        \cdots;
        \mathbf{e}^{a}_{|\mathcal{A}|}
    ]
    \in
    \mathbb{R}^{|\mathcal{A}|\times d_a},
    \label{eq:apb_prompt_bank}
\end{equation}
where each row corresponds to one supported downstream application. Unlike
TPM and DPR, which automatically infer their conditions from the input
representations, APB directly selects the prompt associated with the
user-specified application:
\begin{equation}
    \mathbf{e}^{a}
    =
    \mathbf{E}[a],
    \qquad
    a\in\mathcal{A}.
    \label{eq:apb_selection}
\end{equation}

Let $\widehat{\mathbf{u}}^{t}_{l}$ denote the task-modulated feature produced by TPM. The selected prompt is first projected to the channel dimension of the current decoder level:
\begin{equation}
    \mathbf{p}^{a}_{l}
    =
    P^{a}_{l}
    \left(
        \mathbf{e}^{a}
    \right),
    \qquad
    \mathbf{q}^{a}_{l}
    =
    \operatorname{GAP}
    \left(
        \widehat{\mathbf{u}}^{t}_{l}
    \right),
    \label{eq:apb_projection}
\end{equation}
where $\mathbf{q}^{a}_{l}$ summarizes the current feature state.
In the prompt-injection branch, APB predicts a channel-wise gate from the application prompt and the feature descriptor:
\begin{equation}
    \mathbf{g}^{p}_{l}
    =
    \sigma
    \left(
        W^{p}_{l}
        [\mathbf{q}^{a}_{l};\mathbf{p}^{a}_{l}]
        +
        \mathbf{b}^{p}_{l}
    \right).
    \label{eq:apb_prompt_gate}
\end{equation}
The gated prompt is expanded spatially and transformed into an
application-specific residual:
\begin{equation}
    \mathbf{r}^{p}_{l}=\mathcal{C}^{p}_{l}(( \mathbf{g}^{p}_{l}\odot \mathbf{p}^{a}_{l})
   ),
    \label{eq:apb_prompt_injection}
\end{equation}
where $\mathcal{C}^{p}_{l}$ is a lightweight projection. This branch injects application-relevant priors without directly replacing the fused representation.


To retain the visual evidence produced by DPR and TPM, the
content-retention branch predicts a second gate:
\begin{equation}
    \mathbf{g}^{c}_{l} = \sigma\left(
        \operatorname{MLP}
        [\mathbf{q}^{a}_{l};\mathbf{p}^{a}_{l}]
    \right).
    \label{eq:apb_content_gate}
\end{equation}
The retained content feature is computed as
\begin{equation}
    \mathbf{r}^{c}_{l}=\mathbf{g}^{c}_{l} \odot \widehat{\mathbf{u}}^{t}_{l}+
    (1-\mathbf{g}^{c}_{l}) \odot \mathcal{C}^{c}_{l}(\widehat{\mathbf{u}}^{t}_{l}),
    \label{eq:apb_content_retention}
\end{equation}
where $\mathcal{C}^{c}_{l}$ denotes a lightweight content adapter. The gate dynamically balances the original fusion representation and its application-adapted transformation. The output of APB is obtained by combining prompt injection with retained content:
\begin{equation}
    \mathbf{h}^{a}_{l} = \mathbf{r}^{c}_{l} + \mathbf{r}^{p}_{l}.
    \label{eq:apb_output}
\end{equation}
The resulting feature is passed to the current decoder block and propagated to the next higher-resolution stage. When no downstream application is specified, APB is bypassed and
$\mathbf{h}^{a}_{l}=\widehat{\mathbf{u}}^{t}_{l}$. The two gated branches allow APB to introduce application-discriminative information while limiting undesirable changes to fusion-relevant structures. In this work, APB is instantiated for object detection and semantic segmentation; additional applications can be incorporated by adding new prompt entries and lightweight adaptation parameters without retraining the complete fusion backbone.


\subsection{Training Strategy}
\label{sec:training}
HP-UniIF is optimized in three stages to prevent the three adaptation objectives from interfering with one another.

\paragraph{Stage 1} Multi-Task Fusion Learning.
We first train the latent fusion layer, skip-fusion layers, decoder, and TPM using clean source pairs from all fusion tasks. For task $t$, the fusion objective is written as
\begin{equation}
    \mathcal{L}^{t}_{\mathrm{fus}} =\sum_{m\in\mathcal{M}_{t}}    \lambda^{t}_{m}\mathcal{L}_{m},
    \label{eq:fusion_loss}
\end{equation}

The task-routing loss is
\begin{equation}
    \mathcal{L}_{\mathrm{T}}= -\frac{1}{L} \sum_{l=1}^{L} \sum_{k=1}^{|\mathcal{T}|} y^{t}_{k}\log\omega^{t}_{lk},
\end{equation}
where $\mathbf{y}^{t}$ is the task label available only during training. The Stage-1 objective is
\begin{equation}
    \mathcal{L}_{1}=\mathcal{L}^{t}_{\mathrm{fus}}+ \lambda_{\mathrm{T}}\mathcal{L}_{\mathrm{T}}.
    \label{eq:stage1}
\end{equation}

\paragraph{Stage 2: Degradation-Aware Restoration.}
The Stage-1 fusion network is frozen, and DPR together with the latent control branch is trained using paired clean and degraded samples. Let
$\mathbf{z}^{c}_{0}$ denote the fused latent obtained from the corresponding clean source pair. Because $\mathbf{z}^{d}_{n}$ is generated from the degraded latent, the clean-oriented noise target is defined as
\begin{equation}
    \boldsymbol{\epsilon}^{\star}_{n}=\frac{
    \mathbf{z}^{d}_{n}-\sqrt{\bar{\alpha}_{n}}\mathbf{z}^{c}_{0}
    }{\sqrt{1-\bar{\alpha}_{n}}}.
\end{equation}
The noise-prediction and latent-recovery objectives are
\begin{align}
    \mathcal{L}_{\mathrm{lat}} &=\left\| \widehat{\mathbf{z}}_{0}-
    \mathbf{z}^{c}_{0}
    \right\|_{2}^{2} + \sum^L_{l=0}\lambda_l \left\| \widehat{\mathbf{u}}_{l}-
    \mathbf{h}^{c}_{l}
    \right\|_{2}^{2}.
\end{align}
The degradation-routing loss is denoted by $\mathcal{L}_{\mathrm{D}}$, implemented as cross-entropy for single degradations and a soft-label objective for compound degradations. The Stage-2 objective is
\begin{equation}
    \mathcal{L}_{2} =\lambda_{\mathrm{lat}}
    \mathcal{L}_{\mathrm{lat}} + \lambda_{\mathrm{D}}
    \mathcal{L}_{\mathrm{D}}.
    \label{eq:stage2}
\end{equation}

\paragraph{Stage 3: Application Adaptation.}
Finally, the fusion and restoration paths are frozen. APB and the
corresponding application head are optimized using downstream annotations:
\begin{equation}
    \mathcal{L}_{3}=\mathcal{L}_{\mathrm{app}}
    \label{eq:stage3}
\end{equation}
where $\mathcal{L}_{\mathrm{app}}$ is the detection or segmentation objective.
The fusion-preservation term prevents downstream optimization from discarding source information that remains important for visual fusion.
This stage-wise strategy establishes a clear functional hierarchy: TPM learnshow to fuse different source pairs, DPR learns how to recover corrupted evidence, and APB learns how to adapt the fused representation to a specified application.

==> sec/3_method_bak1.tex <==

\section{Method}
\label{sec:method}
\subsection{Framework Overview}
Given two source images, $\mathbf{x}^{1}$ and $\mathbf{x}^{2}$, the fusion task $t$ and degradation condition $d$ are unknown and are therefore inferred adaptively from the input representations, whereas the downstream application identity $a$ is optionally specified when application-oriented adaptation is required.
\begin{equation}
    \mathbf{y}= \mathcal{G}_{\Theta}
    \left(
        \mathbf{x}^{1},
        \mathbf{x}^{2}; t,
        a
    \right),
    \qquad t\in\mathcal{T},
    a\in\mathcal{A}\cup\{\varnothing\},
    \label{eq:problem_formulation}
\end{equation}
where $t$ denotes the specified fusion-task identity and $a$ denotes the optional downstream application. TPM and APB select task- and application-specific prompts according to $t$ and $a$, respectively, whereas DPR estimates degradation conditions directly from the input representations.

As illustrated in Fig.~\ref{fig:framework}, HP-UniIF is built on a pretrained latent diffusion model comprising a variational autoencoder (VAE) and a denoising U-Net. For each source image, the VAE encoder extracts a latent code together with hierarchical intermediate features:
\begin{equation}
    \left(
        \mathbf{z}^{i},
        \{\mathbf{s}^{i}_{l}\}_{l=1}^{L}
    \right)
    =
    \mathcal{E}(\mathbf{x}^{i}),
    \qquad
    i\in\{1,2\},
    \label{eq:source_encoding}
\end{equation}
where $\mathbf{z}^{i}$ denotes the latent representation and $\mathbf{s}^{i}_{l}$ is the intermediate feature extracted at encoder level $l$.

The source latents are first aggregated through a learnable convolutional projection:
\begin{equation}
    \mathbf{z}^{f}=F_{z}\!\left([\mathbf{z}^{1};\mathbf{z}^{2}]\right)
    \label{eq:latent_fusion}
\end{equation}
where $[\cdot;\cdot]$ denotes channel-wise concatenation. The fused latent $\mathbf{z}^{f}$ is then progressively refined through $T$ denoising steps to yielding the clean latent representation $\mathbf{z}_{0}$. 

Subsequently, $\mathbf{z}_{0}$ is decoded together with the hierarchical source features in a coarse-to-fine manner. The decoding process at level $l$ can be expressed as $\{h_l\}_L=\mathcal{D}(z_0, \{s\}_l^i)$. 

\label{sec:tpm}

\subsection{Task Prompt Modulation}
\label{sec:tpm}

Different fusion tasks require distinct information-selection and
preservation behaviors. For example, infrared--visible fusion emphasizes
cross-modal complementarity, whereas multi-exposure and multi-focus fusion
favor exposure-aware and focus-aware source selection, respectively.
Task Prompt Modulation (TPM) therefore introduces a task-conditioned prompt
that progressively adapts the shared latent and decoder representations to
the current fusion objective.

For each fusion task $t\in\mathcal{T}$, TPM maintains a learnable prompt
embedding:
\begin{equation}
    \mathbf{P}^{T}
    =
    [
        \mathbf{p}^{T}_{1};
        \ldots;
        \mathbf{p}^{T}_{|\mathcal{T}|}
    ]
    \in
    \mathbb{R}^{|\mathcal{T}|\times d_t},
    \qquad
    \mathbf{p}^{T}_{0}
    =
    \mathbf{P}^{T}[t],
    \label{eq:tpm_prompt_initialization}
\end{equation}
where $\mathbf{p}^{T}_{0}$ initializes the task condition and is subsequently
propagated across the latent, decoder, and output stages.

At decoder level $l$, the restored source features produced by DPR are first
fused and combined with the incoming decoder representation:
\begin{equation}
    \mathbf{u}^{T}_{l}
    =
    \mathcal{C}^{f}_{l}
    \left(
        [
            \widetilde{\mathbf{s}}^{1}_{l};
            \widetilde{\mathbf{s}}^{2}_{l}
        ]
    \right)
    +
    \mathcal{U}^{T}_{l}
    \left(
        \mathbf{h}_{l+1}
    \right),
    \label{eq:tpm_feature_aggregation}
\end{equation}
where $\mathcal{C}^{f}_{l}$ performs cross-source skip fusion and
$\mathcal{U}^{T}_{l}$ aligns the incoming decoder feature to the current
spatial resolution.

Rather than using a fixed task embedding throughout the decoder, TPM updates
the prompt according to the current feature state. A compact feature
descriptor is first extracted as
\begin{equation}
    \mathbf{q}^{T}_{l}
    =
    \Phi^{T}_{l}
    \left(
        \operatorname{GAP}
        \left(
            \mathbf{u}^{T}_{l}
        \right)
    \right),
    \label{eq:tpm_feature_descriptor}
\end{equation}
where $\Phi^{T}_{l}$ denotes a lightweight projection. The incoming prompt is
then refined using the feature descriptor and a learnable stage token
$\mathbf{e}^{T}_{l}$:
\begin{equation}
    \mathbf{p}^{T}_{l}
    =
    \mathbf{p}^{T}_{l+1}
    +
    R^{T}_{l}
    \left(
        [
            \mathbf{p}^{T}_{l+1}
            +
            \mathbf{e}^{T}_{l};
            \mathbf{q}^{T}_{l}
        ]
    \right),
    \label{eq:tpm_prompt_refinement}
\end{equation}
where $R^{T}_{l}$ is a prompt-refinement network. This progressive prompt refinement update allows the task condition to evolve from coarse semantic representations to fine-grained spatial details.

The refined prompt predicts channel-wise affine parameters and an injection gate:
\begin{equation}
    \left(
        \boldsymbol{\gamma}^{T}_{l},
        \boldsymbol{\beta}^{T}_{l},
        \mathbf{g}^{T}_{l}
    \right)
    =
    M^{T}_{l}
    \left(
        \mathbf{p}^{T}_{l}
    \right).
    \label{eq:tpm_modulation_parameters}
\end{equation}
The task-adapted feature is obtained through bounded gated residual modulation:
\begin{equation}
    \widehat{\mathbf{u}}^{T}_{l}
    =
    \mathbf{u}^{T}_{l} +\sigma \left(  \mathbf{g}^{T}_{l}    \right)
    \odot
    \left[
        \rho_l
        \tanh
        \left(
            \boldsymbol{\gamma}^{T}_{l}
        \right)
        \odot
        \mathbf{u}^{T}_{l}
        +
        \rho_l
        \tanh
        \left(
            \boldsymbol{\beta}^{T}_{l}
        \right)
    \right],
    \label{eq:tpm_feature_modulation}
\end{equation}
where $\rho_l$ is a small residual scale, and all channel-wise parameters are broadcast along the spatial dimensions. The identity pathway preserves the shared representation, while the bounded affine transformation and sigmoid gate prevent excessive task-specific perturbations.

The same feature-guided modulation is applied to the fused latent before decoding and to the final output representation, with stage-specific parameters and tokens. The updated prompt is passed sequentially across these stages, enabling consistent task conditioning throughout the generation process. Consequently, TPM adapts the shared backbone to different fusion
objectives while retaining a compact and stable task-specific modulation path.



\subsection{Degradation Prompt Router}
\label{sec:dpr}

Input degradations may corrupt source features differently across modalities and spatial scales, making direct skip fusion prone to propagating unreliable information into the decoder. To address this issue, the Degradation Prompt Router (DPR) restores the two source skip features before they are fused at
each decoder level. Specifically, DPR retrieves reusable degradation patterns from a learnable prompt pool and combines them with an input-adaptive prompt to guide gated feature correction.

At decoder level $l$, DPR estimates the degradation condition from the two source skip features and the incoming decoder representation:
\begin{equation}
    \mathbf{a}^{d}_{l}
    =
    \operatorname{GAP}
    \left(
        \mathcal{C}^{d}_{l}
        \left(
            [
                \mathbf{s}^{1}_{l};
                \mathbf{s}^{2}_{l};
                |\mathbf{s}^{1}_{l}-\mathbf{s}^{2}_{l}|;
                \mathcal{U}^{d}_{l}(\mathbf{h}_{l+1})
            ]
        \right)
    \right),
    \label{eq:dpr_descriptor}
\end{equation}
where $\mathcal{U}^{d}_{l}$ aligns the incoming decoder feature with the
current skip features, and $\mathcal{C}^{d}_{l}$ denotes a convolutional
projection. The cross-source discrepancy provides an explicit cue for
modality-dependent corruption, while $\mathbf{h}_{l+1}$ supplies contextual
information from the coarser decoder stage.

DPR maintains a level-specific prompt pool
$\{(\mathbf{k}^{d}_{l,j},\mathbf{p}^{d}_{l,j})\}_{j=1}^{N_p}$.
A normalized query
\begin{equation}
    \mathbf{q}^{d}_{l}
    =
    \operatorname{Norm}
    \left(
        Q^{d}_{l}(\mathbf{a}^{d}_{l})
    \right)
\end{equation}
is used to retrieve the $K$ most relevant prompt entries. The resulting
retrieval prompt is
\begin{equation}
    \mathbf{p}^{r}_{l}
    =
    \sum_{j\in\mathcal{I}_{l}}
    \omega^{d}_{l,j}\mathbf{p}^{d}_{l,j},
    \qquad
    \omega^{d}_{l,j}
    =
    \frac{
        \exp(r^{d}_{l,j}/\tau_d)
    }{
        \sum_{m\in\mathcal{I}_{l}}
        \exp(r^{d}_{l,m}/\tau_d)
    },
    \label{eq:dpr_retrieval}
\end{equation}
where
$r^{d}_{l,j}
=
(\mathbf{q}^{d}_{l})^{\top}
\operatorname{Norm}(\mathbf{k}^{d}_{l,j})$,
$\mathcal{I}_{l}
=
\operatorname{TopK}(\{r^{d}_{l,j}\}_{j=1}^{N_p},K)$,
and $\tau_d$ is a temperature parameter.

To complement the reusable degradation patterns with sample-specific information, DPR generates an input-adaptive prompt and combines it with the retrieved prompt:
\begin{equation}
    \mathbf{p}^{g}_{l}
    =
    G^{d}_{l}(\mathbf{a}^{d}_{l}),
    \qquad
    \mathbf{c}^{d}_{l}
    =
    F^{d}_{l}
    \left(
        [\mathbf{p}^{r}_{l};\mathbf{p}^{g}_{l}]
    \right),
    \label{eq:dpr_prompt_fusion}
\end{equation}
where $\mathbf{c}^{d}_{l}$ encodes both reusable restoration knowledge and
input-dependent degradation characteristics.

Conditioned on $\mathbf{c}^{d}_{l}$, a lightweight restoration transform
predicts a source-specific correction
$\Delta\mathbf{s}^{d,i}_{l}$ and its injection gate
$\mathbf{g}^{d,i}_{l}$. The restored skip feature is written compactly as
\begin{equation}
    \widetilde{\mathbf{s}}^{i}_{l}
    =
    \mathbf{s}^{i}_{l}
    +
    \sigma(\mathbf{g}^{d,i}_{l})
    \odot
    \Delta\mathbf{s}^{d,i}_{l},
    \qquad
    \left(
        \Delta\mathbf{s}^{d,i}_{l},
        \mathbf{g}^{d,i}_{l}
    \right)
    =
    R^{d,i}_{l}
    \left(
        \mathbf{s}^{i}_{l},
        \mathbf{c}^{d}_{l}
    \right),
    \label{eq:dpr_feature_restoration}
\end{equation}
where $R^{d,i}_{l}$ denotes the prompt-conditioned restoration block. The
identity pathway preserves reliable source evidence, while the learned gate
controls how much degradation-aware correction is introduced.

Finally, the two restored skip features are fused and delivered to the
subsequent task-adaptive decoder:
\begin{equation}
    \mathbf{f}_{l}
    =
    \mathcal{C}^{f}_{l}
    \left(
        [
            \widetilde{\mathbf{s}}^{1}_{l};
            \widetilde{\mathbf{s}}^{2}_{l}
        ]
    \right).
    \label{eq:dpr_skip_fusion}
\end{equation}
By operating before skip-feature fusion, DPR suppresses degradation-induced interference while retaining complementary source information for subsequent task-conditioned modulation.


\subsection{Application Prompt Bank}
\label{sec:apb}

APB introduces application-specific adaptation through a compact prompt bank.

We construct a learnable application prompt bank
\begin{equation}
    \mathbf{E}
    =
    [
        \mathbf{e}^{a}_{1};
        \mathbf{e}^{a}_{2};
        \cdots;
        \mathbf{e}^{a}_{|\mathcal{A}|}
    ]
    \in
    \mathbb{R}^{|\mathcal{A}|\times d_a},
    \label{eq:apb_prompt_bank}
\end{equation}
where each row corresponds to one supported downstream application. Unlike
TPM and DPR, which automatically infer their conditions from the input
representations, APB directly selects the prompt associated with the
user-specified application:
\begin{equation}
    \mathbf{e}^{a}
    =
    \mathbf{E}[a],
    \qquad
    a\in\mathcal{A}.
    \label{eq:apb_selection}
\end{equation}

Let $\widehat{\mathbf{u}}^{t}_{l}$ denote the task-modulated feature produced by TPM. The selected prompt is first projected to the channel dimension of the current decoder level:
\begin{equation}
    \mathbf{p}^{a}_{l}
    =
    P^{a}_{l}
    \left(
        \mathbf{e}^{a}
    \right),
    \qquad
    \mathbf{q}^{a}_{l}
    =
    \operatorname{GAP}
    \left(
        \widehat{\mathbf{u}}^{t}_{l}
    \right),
    \label{eq:apb_projection}
\end{equation}
where $\mathbf{q}^{a}_{l}$ summarizes the current feature state.
In the prompt-injection branch, APB predicts a channel-wise gate from the
application prompt and the feature descriptor:
\begin{equation}
    \mathbf{g}^{p}_{l}
    =
    \sigma
    \left(
        W^{p}_{l}
        [\mathbf{q}^{a}_{l};\mathbf{p}^{a}_{l}]
        +
        \mathbf{b}^{p}_{l}
    \right).
    \label{eq:apb_prompt_gate}
\end{equation}
The gated prompt is expanded spatially and transformed into an
application-specific residual:
\begin{equation}
    \mathbf{r}^{p}_{l}=\mathcal{C}^{p}_{l}(( \mathbf{g}^{p}_{l}\odot \mathbf{p}^{a}_{l})
   ),
    \label{eq:apb_prompt_injection}
\end{equation}
where $\mathcal{C}^{p}_{l}$ is a lightweight projection. This branch injects application-relevant priors without directly replacing the fused representation.


To retain the visual evidence produced by DPR and TPM, the
content-retention branch predicts a second gate:
\begin{equation}
    \mathbf{g}^{c}_{l} = \sigma\left(
        \operatorname{MLP}
        [\mathbf{q}^{a}_{l};\mathbf{p}^{a}_{l}]
    \right).
    \label{eq:apb_content_gate}
\end{equation}
The retained content feature is computed as
\begin{equation}
    \mathbf{r}^{c}_{l}=\mathbf{g}^{c}_{l} \odot \widehat{\mathbf{u}}^{t}_{l}+
    (1-\mathbf{g}^{c}_{l}) \odot \mathcal{C}^{c}_{l}(\widehat{\mathbf{u}}^{t}_{l}),
    \label{eq:apb_content_retention}
\end{equation}
where $\mathcal{C}^{c}_{l}$ denotes a lightweight content adapter. The gate dynamically balances the original fusion representation and its application-adapted transformation. The output of APB is obtained by combining prompt injection with retained content:
\begin{equation}
    \mathbf{h}^{a}_{l} = \mathbf{r}^{c}_{l} + \mathbf{r}^{p}_{l}.
    \label{eq:apb_output}
\end{equation}
The resulting feature is passed to the current decoder block and propagated to the next higher-resolution stage. When no downstream application is specified, APB is bypassed and
$\mathbf{h}^{a}_{l}=\widehat{\mathbf{u}}^{t}_{l}$. The two gated branches allow APB to introduce application-discriminative information while limiting undesirable changes to fusion-relevant structures. In this work, APB is instantiated for object detection and semantic segmentation; additional applications can be incorporated by adding new prompt entries and lightweight adaptation parameters without retraining the complete fusion backbone.




\subsection{Training Strategy}
\label{sec:training}
HP-UniIF is optimized in three stages to prevent the three adaptation objectives from interfering with one another.

\paragraph{Stage 1} Multi-Task Fusion Learning.
We first train the latent fusion layer, skip-fusion layers, decoder, and TPM using clean source pairs from all fusion tasks. For task $t$, the fusion objective is written as
\begin{equation}
    \mathcal{L}^{t}_{\mathrm{fus}} =\sum_{m\in\mathcal{M}_{t}}    \lambda^{t}_{m}\mathcal{L}_{m},
    \label{eq:fusion_loss}
\end{equation}

The task-routing loss is
\begin{equation}
    \mathcal{L}_{\mathrm{T}}= -\frac{1}{L} \sum_{l=1}^{L} \sum_{k=1}^{|\mathcal{T}|} y^{t}_{k}\log\omega^{t}_{lk},
\end{equation}
where $\mathbf{y}^{t}$ is the task label available only during training. The Stage-1 objective is
\begin{equation}
    \mathcal{L}_{1}=\mathcal{L}^{t}_{\mathrm{fus}}+ \lambda_{\mathrm{T}}\mathcal{L}_{\mathrm{T}}.
    \label{eq:stage1}
\end{equation}

\paragraph{Stage 2: Degradation-Aware Restoration.}
The Stage-1 fusion network is frozen, and DPR together with the latent control branch is trained using paired clean and degraded samples. Let
$\mathbf{z}^{c}_{0}$ denote the fused latent obtained from the corresponding clean source pair. Because $\mathbf{z}^{d}_{n}$ is generated from the degraded latent, the clean-oriented noise target is defined as
\begin{equation}
    \boldsymbol{\epsilon}^{\star}_{n}=\frac{
    \mathbf{z}^{d}_{n}-\sqrt{\bar{\alpha}_{n}}\mathbf{z}^{c}_{0}
    }{\sqrt{1-\bar{\alpha}_{n}}}.
\end{equation}
The noise-prediction and latent-recovery objectives are
\begin{align}
    \mathcal{L}_{\mathrm{lat}} &=\left\| \widehat{\mathbf{z}}_{0}-
    \mathbf{z}^{c}_{0}
    \right\|_{2}^{2} + \sum^L_{l=0}\lambda_l \left\| \widehat{\mathbf{u}}_{l}-
    \mathbf{h}^{c}_{l}
    \right\|_{2}^{2}.
\end{align}
The degradation-routing loss is denoted by $\mathcal{L}_{\mathrm{D}}$, implemented as cross-entropy for single degradations and a soft-label objective for compound degradations. The Stage-2 objective is
\begin{equation}
    \mathcal{L}_{2} =\lambda_{\mathrm{lat}}
    \mathcal{L}_{\mathrm{lat}} + \lambda_{\mathrm{D}}
    \mathcal{L}_{\mathrm{D}}.
    \label{eq:stage2}
\end{equation}

\paragraph{Stage 3: Application Adaptation.}
Finally, the fusion and restoration paths are frozen. APB and the
corresponding application head are optimized using downstream annotations:
\begin{equation}
    \mathcal{L}_{3}=\mathcal{L}_{\mathrm{app}}
    \label{eq:stage3}
\end{equation}
where $\mathcal{L}_{\mathrm{app}}$ is the detection or segmentation objective.
The fusion-preservation term prevents downstream optimization from discarding source information that remains important for visual fusion.
This stage-wise strategy establishes a clear functional hierarchy: TPM learnshow to fuse different source pairs, DPR learns how to recover corrupted evidence, and APB learns how to adapt the fused representation to a specified application.
